This Person (Probably) Exists. Identity Membership Attacks Against GAN Generated Faces

Recently, generative adversarial networks (GANs) have achieved stunning realism, fooling even human observers. Indeed, the popular tongue-in-cheek website {\small \url{ http://thispersondoesnotexist.com}}, taunts users with GAN generated images that seem too real to believe. On the other hand, GANs do leak information about their training data, as evidenced by membership attacks recently demonstrated in the literature. In this work, we challenge the assumption that GAN faces really are novel creations, by constructing a successful membership attack of a new kind. Unlike previous works, our attack can accurately discern samples sharing the same identity as training samples without being the same samples. We demonstrate the interest of our attack across several popular face datasets and GAN training procedures. Notably, we show that even in the presence of significant dataset diversity, an over represented person can pose a privacy concern.

==> 1_intro_old.tex <==
\section{Introduction}

Among the recent advances of deep learning, Generative Adversarial Networks (GANs)\cite{goodfellow2014generative} are arguably the most burgeoning area of research.
This is evidenced by their rich applications such as ageing, inpainting, super-resolution, or attribute modification \cite{ledig2017photo,yu2018generative,webster2019detecting,choi2018stargan}. 
Less studied lines of research include measuring the statistical consistency between the generated distribution and the real one \cite{heusel2017gans,sajjadi2018assessing,simon2019revisiting}, or in theoretical analysis of the GAN learning problem \cite{arora2017generalization}. 



\newlength{\malongueur}
\setlength{\malongueur}{.3\linewidth}
\begin{figure}

    \centerline{\em Samples from a GAN $G$ trained with a dataset $\mathcal{D}_G$ composed of $\yg$ distinct identities}
    \vspace{2mm}
    
    \centering
    \begin{tabular}{c c}
    \multicolumn{2}{c}{(a) $|\yg| = 220$}
    \\
    \includegraphics[height=\malongueur]{figures/teaser/Teaser_Setting1_40Id_generated.jpg}
    &
    \includegraphics[height=\malongueur]{figures/teaser/Teaser_Setting1_40Id_training.jpg}
    \\
    $G(z)$ & $x \in \mathcal{D}_G$
    %$x = G(z)$ & $y \in \mathcal{D}_G$ s.t. $Id(y) = Id(x)$
    \end{tabular}
    %
    \hfill
    %
    \begin{tabular}{c c}
    \multicolumn{2}{c}{(b) $|\yg| = 440$}
    \\
    \includegraphics[height=\malongueur]{figures/teaser/Teaser_Setting1_440Id_generated.jpg}
    &
    \includegraphics[height=\malongueur]{figures/teaser/Teaser_Setting1_440Id_training.jpg}
    \\
    $G(z)$ & $x \in \mathcal{D}_G$
    \end{tabular}
    %
    \hfill
    %
    \begin{tabular}{c c}
    \multicolumn{2}{c}{(c) $|\yg| = 2020$}
    \\
    \includegraphics[height=\malongueur]{figures/teaser/Teaser_Setting2_20Id_generated.jpg}
    &
    \includegraphics[height=\malongueur]{figures/teaser/Teaser_Setting2_20Id_training.jpg}
    \\
    $G(z)$ & $x \in \mathcal{D}_G$
    \end{tabular}
    
    
    
    \caption{
    %\textbf{Have you already seen this person?} 
    \textbf{These people appear to exist.} 
    \em Each row displays a GAN generated image (left) with three training images (right) having the same predicted identity. 
    Images are generated with StyleGAN~\cite{karras2019style} using $N$ training images (respectively 40k, 80k and 46k) from \VGGFace2 and identified with a face identification network.
    %
    We investigate two different scenarios in this paper: in (a) and (b) identities are evenly distributed over the datasets, where in (c) a small subset is more represented. 
    %
    While some samples merely bear resemblance, other generated images strongly share idiosyncratic features of training identities. Such a nearest neighbor search helps factor out the ways in which GANs can generalize (via pose, lighting and expression) and elucidate overfitting on identities. This is a threat to privacy as we demonstrate in our blind identity membership attack. % (see paper).
    }
    \label{fig:teaser}
\end{figure}

It is fairly clear GANs have made incredible progress in terms of visual quality, as measured by the popular Frechet Inception Distance (FID) \cite{heusel2017gans}, or merely by sample inspection (for example, see StyleGAN samples in Fig.~\ref{fig:teaser}). However, it remains unclear in what ways GANs generalize. Several works have noted that the GAN \textit{discriminator} tends to overfit the training set \cite{arjovsky2017wasserstein,brock2018large}, in the sense that it will label hold out test images as fake. Such an observation was used to exploit the privacy of GANs in the LOGAN approach \cite{hayes2019LOGANMembershipInference}. Nonetheless, the LOGAN leak only involves the discriminator in a direct way, leaving the generator in a gray area. In fact, several heuristics exist to show GANs do in fact produce novel data, whether it be by sample interpolation and attribute modification  as demonstrated in the first GAN works \cite{goodfellow2014generative,radford2015unsupervised}, or by the ability of GANs to generalize to novel pose and expression \cite{shen2018faceid}. Furthermore, a general belief is that the generated images are always entirely original (in terms of identity), as can be testified by the popular website
{\small \url{https://thispersondoesnotexist.com/}}.


\paragraph{\bf GANs and Privacy}
In addition to the theoretical interest of GAN generalization, several new works have evaluated the privacy of generative models.
Some recent works raise the possibility of applying various privacy mechanisms during GAN training \cite{xie2018differentially,jordon2019PATEGANGeneratingSynthetic}. Unfortunately, so far the proposed approaches have failed to reach a satisfactory trade-off between the theoretical privacy guarantees and the quality of the generated distributions. That is, for any satisfying privacy guarantee, these methods are unable to generate even low quality data. Still, such an approach is highly sought after, as it would allow for the release of private data via synthetic surrogates, e.g. in medicine where data can not be made public. 


Empirically, however, it has been observed that GANs do in fact show some form of privacy \cite{webster2019detecting,webster2019generating}. 
For example, \cite{webster2019detecting} builds on a latent recovery mechanism to characterize overfitting. GAN generators appear to be able to generate samples from test and train sets equally well, making them at least somewhat robust against membership attacks, described next.



\paragraph{\bf Membership attacks} Neural networks leak information in numerous ways about the data on which they are trained  \cite{song2017MachineLearningModels,carlini2019SecretSharerEvaluating}. Often times training data is private or copyrighted, which effects the utility of the model as it can be prone to attackers seeking information on the training set. Amongst the most well known attacks are the \textit{membership inference attacks} \cite{shokri2017MembershipInferenceAttacks}. In this type of attack, an attacker tries to discern which samples were used during model training. In \cite{shokri2017MembershipInferenceAttacks}, training set samples could be nearly perfectly determined from model outputs on the MNIST classification task. Such an attack typically utilizes statistics of the model output. For example, a model that overfits will have low values of the loss function on the training samples, thus allowing for a simple thresholding attack. Similar attacks can be seen in \cite{melis2018InferenceAttacksCollaborative,fredrikson2015ModelInversionAttacks,melis2019ExploitingUnintendedFeature}.
\iffalse
% \juju{we need to cite \cite{sablayrolles2019white} here :}
It is shown additionally in \cite{sablayrolles2019white} that optimal strategies for such type of attacks on classification networks merely depend on the loss function used during training. As a consequence, \emph{black-box} attacks (where only the architecture of the network is known) can perform as good as \emph{white-box} attacks where parameters of the networks are known as well.
Furthermore, \cite{sablayrolles2019white} elucidates a fundamental relationship between differential privacy (DP) and membership attacks, showing that membership attacks become impossible with a strong enough DP privacy.
\fi

More recently, membership attacks have been devised against generative models \cite{liu2018PerformingCoMembershipAttacks,hayes2019LOGANMembershipInference}. These attacks are slightly more intuitive, in the sense that generated samples leave in the same space as the data, and they may be visually similar or identical to exact training samples. In \cite{webster2019detecting}, the non-adversarial procedure of GLO \cite{bojanowski2018OptimizingLatentSpace}  reproduces some training samples verbatim, while not being able to reproduce test samples coming from the same distribution. 
Such direct leaks were not observed for typical GANs.
However, generated images can resemble training samples in even more subtle ways, as seen in Fig.~\ref{fig:teaser}: generated samples can highly resemble exact identities, even if the images themselves are quite different. 



%Observing that adversarial training procedure combined with high model complexity encourage a distribution of generated examples concentrated around training samples, several researcher introduced explicit privacy mechanisms in the GAN framework. Amongst the two most popular are DP-GAN \cite{xie2018DifferentiallyPrivateGenerative}, which introduced carefully calibrated noises in the training procedure, and  PATE-GAN \cite{jordon2019PATEGANGeneratingSynthetic} relying on differential privacy and federated learning. However, no one has succeeded so far in generating realistic images with privacy guarantees, as the constraints imposed by differential privacy are very strict.

In this context, measuring to which extent modern GANs leak information on the training examples is a matter of importance and has been studied in several papers. Of particular relevance to this work is LOGAN \cite{hayes2019LOGANMembershipInference}, a GAN discriminator separating real and fake images is re-trained on generated images to separate training and test examples, and used to detect training examples. While effective, LOGAN \cite{hayes2019LOGANMembershipInference} assumes to have a set of \textbf{exact} training samples, as well as which percentage of this set is training examples. This information would likely not be known by an attacker. 


\paragraph{\bf Face Generation}
In this work, we focus on GANs trained on facial image data.
Face image datasets are amongst the most popular for demonstrating GAN efficacy, partly because the human eye is particularly attuned to detect artifacts in these images and due to the wide availability of high quality face datasets \cite{kemelmacher2016megaface,cao2018vggface2,liu2018large}. Face datasets include some form of bias in regard to the real distributions of faces.
For instance, datasets are frequently composed of a decent number of instances of the same person (see Fig. \ref{fig:histogram_identity_datasets}).
Besides in some datasets \cite{wang2018deep}, the number of instances per identity is highly versatile (e.g. in MEGAFACE \cite{kemelmacher2016megaface} it ranges from 3 to 2k). One should also note that datasets dedicated to generation such as FFHQ \cite{karras2019style} may well display similar biases due to the lack of any specific safeguard. 


\begin{figure}[htb]
    \centering
    \begin{tabular}{ccc}
    % trim=left bottom right top, clip
    \includegraphics[width=.285\linewidth]{figures/vggf2_identity_histogram_crop.jpg}
    & \includegraphics[width=.29\linewidth]{figures/casia_identity_histogram_crop.jpg}
    & \includegraphics[width=.33\linewidth, trim=0 0 0 110, clip]{figures/celeba_identity_freq.jpg}  \\
         
    \vspace*{1mm}
    \VGGFace2 &  \CASIA & CelebA
    \end{tabular}
    
    \caption{\textbf{Histogram of number of instances per identity for different datasets (\VGGFace2, \CASIA \& CelebA).} 
    \em Far from being uniform, face recognition datasets include bias in terms of the number of examples per identitiy. VGGFace2 was designed to be balanced in this sense, compared here to the \CASIA containing bias in some samples.
    }
    \label{fig:histogram_identity_datasets}
\end{figure}


\paragraph{\bf Identity Membership Attacks} The main contribution of this paper is to provide a membership attack in the blind setting. The membership attacks introduced thus far are able to discern exact instances of training samples. The proposed attack assumes an attacker is trying to discern whether a given \textit{facial identity}, was used during training, which we refer to as a Identity Membership Attack. In this way, the attack should be robust to pose, expression and other variations within the intra-identity images. The proposed identity membership attack does not require the knowledge of training set identities or exact data samples. Rather, an attacker only needs a face classification system. To mark the distinction with the standard, we will refer to the latter as a {\em blind} membership attack. 
Indeed, GANs typically automatically disentangle attributes, and therefore the attack must be robust to variations in pose, expression, etc. Luckily, a well trained face recognition system, especially those trained on challenging datasets, \emph{e.g.} the \VGGFace2 dataset (Fig.~\ref{fig:histogram_identity_datasets}), are well equipped to handle such variations. 

Finally, we would like to highlight that current GAN evaluations are ill equipped for privacy. The FID for example, will not distinguish models which merely reproduce their training set. A similar thing can be said about Inception score \cite{salimans2016improved}, and other GAN evaluation techniques \cite{borji2019pros}, which tend to focus solely on image quality.

The current art, the LOGAN membership attack \cite{hayes2019LOGANMembershipInference}, will not succeed in our setting for two reasons, (1) it was shown not to be effective when it does not have access to training samples (an assumption we make) and (2) it would have to be adapted to the classification setting. 


\paragraph{\bf Outline}
The rest of the paper is organized as follows.
In Section~\ref{sec:protocol} we expose the proposed protocol used to train the face detection network, to perform the attack and to evaluate its performance.
This protocol is tested in Section~\ref{sec:attack} on various datasets (\CASIA and \VGGFace2) with different GANs (StyleGAN and LSGAN) across different attack scenarios.
Performance curves and visual evidence are provided to show membership attacks can be highly successful against GANs even in the blind scenario, and when diverse training data is used.
A discussion and perspectives on future work are given in Section~\ref{sec:conclusion}.
Reviewers will also find additional results in the supplementary material.

%In what follows, we shall describe a simple yet effective attack of such kind. 

%More precisely, we shall see that it performs well when small sets of identities are used, or a small set is over represented.







%In order to conduct our study, we focus on the VGGFace2 dataset \cite{cao2018vggface2}, trained with various GANs, namely StyleGAN \cite{karras2019style}. VGGFace2 is appealing because of a balanced image per identity histogram, which allows for careful control of the diversity of the training set. In this way we are able to simulate varying amounts of bias that may be present in other datasets.  The contributions of this work are as follows:
%\begin{enumerate}
    %\item In Section~\ref{sec:protocol}, we introduce a novel GAN evaluation procedure. First we control the identities a GAN sees during training and subsequently GAN innovation is  measured statistically using a face identification network. Importantly, we demonstrate GANs do tend to produce training identities, even with moderate to large dataset sizes.
    %\item In Section~\ref{sec:protocol} we use our methodology to  provide additional visual proof corroborating our statistical findings, shown in Fig.~\ref{fig:teaser} and Fig.~\ref{fig:NN_comparison}.
    %\item Finally, in Section~\ref{sec:attack}, we demonstrate a novel membership identity attack. In particular, we use the entropies of the face identification network to discern training identities. Contrary to most membership attack in the literature, this is a pure \emph{black-box} attack.
%\end{enumerate}

%\ryan{perhaps put small table / figure showing characteristics of FAce datasets as in VGGFace2 paper. For example the Images / Identity hostograms.} done below





